Learning Multi-Scale Representations for Material Classification

The recent progress in sparse coding and deep learning has made unsupervised feature learning methods a strong competitor to hand-crafted descriptors. In computer vision, success stories of learned features have been predominantly reported for object recognition tasks. In this paper, we investigate if and how feature learning can be used for material recognition. We propose two strategies to incorporate scale information into the learning procedure resulting in a novel multi-scale coding procedure. Our results show that our learned features for material recognition outperform hand-crafted descriptors on the FMD and the KTH-TIPS2 material classification benchmarks.

==> method.tex <==
%\section{Multi-Scale Spike-and-Slab Sparse Coding (MS4C)}
\section{Multi-Scale Feature Learning Framework}
While we have seen broad application and success of feature learning techniques in object recognition, material recognition still relies on hand-crafted features. The appearance of material classes seem special in many ways. First of all, the samples seem to obey a stronger manifold assumption, as the appearance varies rather smoothly w.r.t. changes in lighting direction, orientation and scale. For objects, more drastic changes can occur due to the more pronounced 3d structure.

In this section, we first describe the commonly used framework for feature learning and then summarize several models we investigated for our tasks. Afterwards, we extend the model for multi-scale feature learning with two different strategies.

\subsection{Unsupervised Feature Learning}
A commonly used patch-based unsupervised feature learning framework is illustrated in Figure ~\ref{fig:pipeline} where one first extract random patches $\{x_1,...,x_n\}$ from training images and learn a feature mapping $f$ (dictionary learning). Once the model is obtained, one can encode the equally spaced sub-patches covering the input image and pool the codes together to form the final feature representation (feature extraction). By altering the model used for feature mapping, we can get different feature representations.

\begin{figure}
\begin{center}
\label{fig:pipeline}\includegraphics[width=8.5cm]{figures/pipeline.png}
\end{center}
\caption{Pipeline for unsupervised feature learning framework.}
\end{figure}

\paragraph{Sparse Coding (SC)}
Sparse coding was originally proposed by Olshauen and Field \cite{olshausen1996emergence} as an unsupervised learning models of low-level sensory processing in humans. More recently, it was used in the self-taught learning framework \cite{raina2007self}. In the first phrase, the dictionary $D$ (also known as basis) is obtained by optimzing:

\begin{eqnarray*}
\begin{aligned}
& \underset{D,s_i}{\text{minimize}}
& & \sum_i \|x_i - D s_i\|_2^2 + \beta \|s_i\|_1 \\
& \text{subject to}
& & \|D_j\|_2 \leq 1, \forall j 
\end{aligned}
\end{eqnarray*}

Then in the next phase, feature representation $s_i$ for each input $x_i$ is obtained by solving the same form of optimization problem but with the learned dictionary.   

\paragraph{Auto-Encoder (AE)}
Auto-encoder is another popular model widely used for learning feature representations in deep learning community. In the first phase, $x$ is first mapped into latent representation $s$ (encoding) with a nonlinear function $s = f(D x + b)$ such as the sigmoid and then mapped back into a reconstruction $z$ through a similar transformation: $z = f(D's + b')$, the dictionary ( or weights) $D$ is obtained by optimizing the reconstruction error. Then during encoding phase, one can easily compute the features through the nonlinear function $f$.

\paragraph{ Spike-and-Slab Sparse Coding (S3C)}
Spike-and-Slab Sparse Coding (S3C) by Goodfellow at el \cite{Goodfellow+etal12:s3c} has been recently proposed to combine the merits of feature learning methods like sparse coding and RBMs. 

The model is a two-layer generative process: the first layer is a  real-valued $D$-dimensional visible vector $v\in R^D$, where  $v_d$ corresponds to the pixel value at position d; the second layer consists of two different kinds of latent variables, the binary \emph{spike} variables $h\in\{0,1\}^N$, the real-valued \emph{slab} variables $s\in R^N$. The spike variable $h_i$ gates the slab variable $s_i$, and those two jointly define the $i^{th}$ hidden unit as $h_i s_i$. The process can be more formally described as follows: 
\begin{eqnarray*}
\forall i \in \{1,...,N\},d\in\{1,...,D\}\\
p(h_i=1)=\sigma(b_i)\\
p(s_i|h_i)=N(s_i|h_i\mu_i,\alpha_{ii}^{-1})\\
p(v_d|s,h)=N(v_d|W_{d:}(h \circ s),\beta_{dd}^{-1})\\
\end{eqnarray*}

\begin{figure}
\begin{center}
\label{fig:figures/s3c_illustration.png}\includegraphics[width=6.5cm]{figures/s3c_illustration.png}
\end{center}
\caption{Graphical illustration of S3C model, where $v_d$ denotes visible units, $h_i$ and $s_i$ represent hidden variables (spike and slack variables respectively), directed arrows stand for dependency.}
\end{figure}
where $\sigma$ is the logistic sigmoid function, $b$ is a set of biases on the spike variables, $\mu$ and $W$ govern the linear dependence of $s$ and $h$ and $v$ on $s$ respectively, $\alpha$ and $\beta$ are diagonal precision matrices of their respective conditionals, $h\circ s$ denotes the element-wise product of $h$ and $s$ and $W_{d:}$ stands for the $d_{th}$ row of the weight matrix $W$ of which each component $W_{di}$ weights the product $h_i s_i$. Columns of $W$ is constrained to have unit norm, $\alpha$ is restricted to be a diagonal matrix and $\beta$ to be a diagonal matrix or a scalar. In particular, W can be interpreted as a series of filters which can be used sparsely to represent the data.

The  model has shown to perform superior to previous feature learning technique and is the best performer on a recent transfer learning challenge where one train the model over the patches from the limited number of training images and a large number of unlabeled image data and then coded both training data and test data with the learned model, a standard linear SVM was then used for classification on the learned representation of data.

As discussed by the S3C's author, one drawback of sparse coding is that the latent variables are not only encouraged to be sparse, but also to be close to 0 when activated. To tackle this issue, the S3C model introduces separate priors to control the activation of units and the magnitude of activated units separately. Though a similar structured RBM model known as $\mu-ssRBM$ \cite{courville2011unsupervised} is also proposed for feature learning, the non-factorial posterior of S3C model can grant better discriminative capability by selectively activating only a small set of features for a given input.   

As we will show qualitatively as well as quantitatively, it seems particularly well suited to capture the data distribution of natural materials and also outperforms the other models in our experiments.

\paragraph{Model Learning}
The variational EM \cite{saul1996exploiting} algorithm is used for model learning. It is a variant of the EM algorithm with modification in the E-step where we only compute a variational approximation to the posterior rather than the posterior itself. In detail, the variational E-step maximizes the energy functional with respect to a distribution $Q$ by minimizing the Kullback-Leibler divergence: $D_{KL}(Q(h,s)||P(h,s|v))$, where $Q(h,s)$ is drawn from a restricted family of distributions to ensure that $Q$ is tractable.

\subsection{Multi-scale Feature Learning}
\paragraph{Importance of Scale Information}
The scale information is a critical element for material and texture recognition problem. 
\cite{caputo05} showed that explicit treatment of scale is necessary for material recognition in realistic settings.
In \cite{Li2012}, Li et al performed a manifold alignment with respect to scale between real and synthesized data, which turned out to be crucial for using the generated data to improve recognition rate. Similarly, local descriptors like LBP are usually limited by their small spatial support area, several extensions \cite{Ojala2002}, \cite{maenpaa2003multi} for multi-scale descriptor have also been shown to overcome the limitation to some extent.  Therefore we propose two different strategies to employ multi-scale information in feature learning:

\begin{figure}
\begin{center}
\label{fig:figures/ss3c.png}\includegraphics[width=8.5cm]{figures/ss3c.png}
\label{fig:figures/js3c.png}\includegraphics[width=8.5cm]{figures/js3c.png}
\end{center}
\caption{Multi-scale feature learning with: multi-scale stacked feature learning (top), multi-scale joint feature learning (bottom).}
\end{figure}

%\begin{figure}
%\begin{center}
%\label{fig:figures/multi-scale_illustration.png}\includegraphics[width=9cm]{figures/multi-scale_illustration.png}
%\end{center}
%\caption{Multi-scale feature learning with: multi-scale collaborated representation (left), multi-scale joint representation (right).}
%\end{figure}

\paragraph{1) Multi-scale Stacked Feature Learning}
In the first strategy, we perform the encoding at multiple scales and stack the obtained codes as a new piece of code, then use this code for classification. In practice, we alter the patch size during encoding for each scale to realize features for multiple spatial resolutions in order to represent the scale information. 

\paragraph{2) Multi-scale Joint Feature Learning}
In the second strategy, we first construct a multi-scale pyramid for each image, apply the feature learning directly on the pyramid and then use the obtained codes for classification. In particular, for color images, we first convert them into gray-scale representation, and then stack its Gaussian pyramid for feature learning. Simultaneously, we perform an additional encoding process on the original image to account for the color information, and together with codes from the gray-scale pyramid representation, we get a complete multi-scale joint representation.
